Solving Discounted Stochastic Two-Player Games with Near-Optimal Time and Sample Complexity

In this paper, we settle the sampling complexity of solving discounted two-player turn-based zero-sum stochastic games up to polylogarithmic factors. Given a stochastic game with discount factor $\gamma\in(0,1)$ we provide an algorithm that computes an $\epsilon$-optimal strategy with high-probability given $\tilde{O}((1 - \gamma)^{-3} \epsilon^{-2})$ samples from the transition function for each state-action-pair. Our algorithm runs in time nearly linear in the number of samples and uses space nearly linear in the number of state-action pairs. As stochastic games generalize Markov decision processes (MDPs) our runtime and sample complexities are optimal due to Azar et al (2013). We achieve our results by showing how to generalize a near-optimal Q-learning based algorithms for MDP, in particular Sidford et al (2018), to two-player strategy computation algorithms. This overcomes limitations of standard Q-learning and strategy iteration or alternating minimization based approaches and we hope will pave the way for future reinforcement learning results by facilitating the extension of MDP results to multi-agent settings with little loss.

==> lower_bound.tex <==

\section{Complexity Lower Bound for Policy and Strategy Iteration}


In this section, we establish complexity lower bounds for strategy iteration and we show that the minimal number of policy evaluations needed to achieve certain accuracy. The lower bounds suggest that the flux ratio is the central quantity that determines the complexity for solving MDP and stochastic games \sidford{way to strong a statement I think, at most it might govern policy / strategy iteration.}.

\subsection{Lower Bound for Policy Iteration}

We first study the complexity of policy iteration for the Markov decision problem, which is a special case of the two-player stochastic game. 
We show that PI needs at least $\Omega(\delta_{\max}/\delta_{\min})$ number of policy evaluations to get an $\epsilon$-optimal policy.
%\lin{Note to self: make sure every place the notation for $M$ is the same.}
\begin{theorem}
	\label{thm:pi-hard}
	There exists an MDP instance $(\cS,\cA,\bP, \br,\gamma)$ with flux ratio $\delta_{\max}/\delta_{\min}$ and an initial policy $\pi^{(0)}$, such that 
	PI takes at least $\Omega(\delta_{\max}/\delta_{\min})$ iterations to obtain a $0.1$-optimal policy.
	%\mw{is 0.1 relative or additive? for a particular $\gamma$? or $\gamma$ sufficiently close to 1?}
\end{theorem}


\paragraph{Hard instance of MDP (HI1)}
To prove the theorem, we first show the hard instance.
Consider an MDP with $T$ states $i=1,2, \ldots, T$.
Let $S$ be an integer with $S'=\Theta(\sqrt{T}) <\sqrt{T}$.
For each state $i\in[T-S'-1]\cup\{T\}$, let there be only one action denoted by $U$.
For each state $i\in [T-S', T-1]$, let there be two actions, the $R$ (right) action and the $U$ (uniform) action. The $R$ action moves the state to its rightward neighbor and the $U$ action transitions the state to a random state uniformly.
%For state $T$, there is only one action $B$.
Therefore, for $i\in[T-S'-1, T]$, $P(i+1|i, R)=1$, and for $i,i'\in [T]$ we have $P(i'|i, U) = 1/T$.
All the rewards are $0$, i.e. $\br(i,U)=\br(i,R) =0$ for $i\in[T-1]$, except for the rightmost reward $r_T:=\br(T, U) = 1$.
\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{hardcase.png}
\caption{The hard MDP instance for policy iteration to correct one action at a time.}
\end{figure}
%\paragraph{Ergodicity}
Let us consider two extreme policies, which we denote by $\pi^e$ and $\pi^0$.
The policy $\pi^0$ is to choose action $U$ at every state.
The policy $\pi^e$ is to choose $R$ action whenever it is possible, i.e., at every state $i$ such that $T-S'\le i<T$.
The transition probability matrix of these policies are
\[
\bP_{\pi^0} = \left[
\begin{array}{cccc}
1/T& 1/T& \ldots& 1/T\\
1/T& 1/T& \ldots& 1/T\\
&&\ldots&\\
1/T& 1/T& \ldots& 1/T
\end{array}
\right]
\quad\text{and}
\quad
\bP_{\pi^e} = \left[
\begin{array}{cccccc}
1/T& 1/T& \ldots& 1/T&1/T& 1/T\\
&& \textcolor{gray}{(T-S' - 1\text{ rows})} &&\\
1/T& 1/T& \ldots& 1/T& 1/T&1/T\\
0&  \ldots & 1 & 0 &0&\ldots\\
0&  \ldots & 0 & 1 &0&\ldots\\
0&  \ldots & 0 & 0 &1&\ldots\\
&&\ldots&&\\
0&0&\ldots & 0&0& 1\\
1/T& 1/T& \ldots&1/T&1/T& 1/T
\end{array}
\right].
\]
Let $\be$ and $\blambda$ be the stationary distributions of the two policies such that  \[
\bP_{\pi^0}^\top \be = \be\quad\text{and}\quad \bP_{\pi^e}^\top\blambda = \blambda.
\]
They admit closed-form expressions as follows
\[
\be = [1,1,1\ldots, 1]^\top/T \quad\text{and}\quad
\blambda = [1, 1, 1,\ldots, 1,2, \ldots, S', S'+1]^\top/\big[T-S'-1 + (S'+1)(S'+2)/2\big].
\]
All other policies will generate stationary distributions that are somewhat ``in between'' $\be$ and $\blambda$, so that the ergodicity ratio of the constructed MDP instance is of the order $\sqrt{T}$. This is proved in the following Lemma \ref{lemma:ergodicity}. 

%\textcolor{red}{In fact the eigenvalue with the largest entry is $\Theta(1/\sqrt{T})$, achieved when $\lambda_{\pi}=\mathrm{normalize}(T/(T-\sqrt{T}+1), T/(T-\sqrt{T}+1), \ldots, T/(T-\sqrt{T}+1), 1, 2, 3, \ldots, \sqrt{T}-1, T/(T-\sqrt{T}+1))$ }

\begin{lemma}
	\label{lemma:ergodicity}
	For any policy $\pi$, let $\blambda_\pi$ be the invariant distribution for the above MDP instance.
	Then there exits $T$ and $S'=\Theta(\sqrt{T})$ such that for any $\pi$, 
	\[
	1/(2T) \le \blambda_\pi(i) \le (S'+1) /T,\qquad i =1,\ldots,T.
	\]
	Therefore the ergodicity ratio of the constructed MDP instance satisfies
\[
c_{\max}/ c_{\min} \lesssim S' = \Theta(\sqrt{T}).
\]
	%for some constants $c, C$.
\end{lemma}
\begin{proof}%\mw{needs work}
	First, we show the upper bound for $\blambda_\pi$.
	We claim that for any policy $\pi$, 
	\[
	\blambda_{\pi}(i)\le \frac{1}{T} \quad\text{for} \quad i\in [T-S'] \cup \{i:~ \pi(i-1) \neq R\}.
	\]
	%$\blambda_{\pi}(i)\le 1/T$ for all $i\le T-\sqrt{T}$ and those $i$ with $\pi(i-1) \neq R$. 
%	Indeed, the stationary distribution satisfies
%	\[
%	\blambda_{\pi}(i) = \sum_{j=1}^{T}\blambda_{\pi}(j) \bP(i|j, \pi(j))
%	\]
	Indeed, for each $j\in [T]$, we have
	\[ 
	\bP\big[i|j, \pi(j)\big] = \left\{\begin{array}{ccc}
	1/T &\text{for} & \pi(j)=U\\
	0 & \text{otherwise} & 
	\end{array}\right.
	\]
	therefore \[
	\blambda_{\pi}(i) =\sum_{j=1}^T\blambda_{\pi}(j) \bP(i|j, \pi(j)) \le 1/T,
	\]
	as desired.
	
	Next, for each $i\in \{j: \pi(j-1) = R\}$, let $s_i$ be the {\it leftmost} state such that $\pi$ chooses action $R$ in a chain of states $ s_i, s_i+1, \ldots, i-1$, i.e.,
	\[
	s_i = \min\{i'< i:\pi(i') = \pi(i'+1) =\ldots \pi(i-1) = R\}.
	\]
	We have $i-s_i \le S'$ since any policy can pick action $R$ for at most $S'$ states.
	Let $n_i = i - s_i$, and we claim that
	\[
	\blambda_{\pi}(i)\le (n_i + 1) / T.
	\]
	We prove this claim by induction on $n_i$.
	For $n_i = 1$, we have $\pi(i-1) = R$ and $\pi(i-2) = U$. 
	Recall that $\blambda_{\pi}(i-1) \le 1/T$ as shown in the last claim.
	We have,
	\[
	\blambda_{\pi}(i) = \blambda_{\pi}(i-1) + 
	\sum_{j\neq i-1}\blambda_{\pi}(j) \bP(i|j, \pi(j))
	\le \blambda_{\pi}(i-1) + 1/T\le 2/T,
	\]
	where the second inequality holds since $\bP(i|j, \pi(j)) =0$ or $1/T$ for all $j\neq i-1$. 
	Suppose for $n_i = k-1$ the claim holds.
	Then for $n_i=k$, we have,
	\begin{align*}
	\blambda_{\pi}(i) &\le \blambda_{\pi}(i-1) + \sum_{j\neq i-1}\blambda_{\pi}(j)\bP(i|j,\pi(j)) \le k / T + 1/T\le (k+1)/T,
	\end{align*}
	as desired.
	
	Next, we show the lower bound.
	We denote an \emph{$R$-chain} in a policy $\pi$  as a tuple $(i', i)$ with $T-S'\le  i'< i<T$ such that
	\[
	\pi(i'- 1) = U,\quad
	 \pi(i') = \pi(i'+1)=\ldots \pi(i-1) = R,\quad \text{and}\quad \pi(i) = U. 
	\]
	Namely, the states $\{i', i'+1, \ldots, i\}$ form a maximal connected component by action $R$.
	In an $R$-chain $(i', i)$, we call $i'$  the \emph{source}, $i$  the \emph{end}, and $i-i'$  the \emph{length}.
	Suppose $\pi$ has $k$ $R$-chains. 
	Let these $R$-trains be $(s_1, s_1+l_1), (s_2, s_2+l_2), \ldots (s_k, s_k+l_k)$.
	%Denote their length as $l_1, l_2, \ldots, l_k$.
	Let 
	\[
	A := \{s_i: i\in [k]\} \cup \{j: j\text{ is not on an $R$-chain}\}
	\]
	We observe that every $i\in A$ is identical in terms of probability transition from other states into $i$.  %the value $\blambda_{\pi}(i')$s are the same.
	Therefore, they must have the same probability in the invariant distribution $\blambda_{\pi}$. 
	%Denote the set of these states as $A$.
	%Recall that $\blambda_{\pi}(s_i) \le 2/T$ for each $i\in[k]$.
	We then have, for every $s\in A$,
	\begin{align*}
	1&=\sum_{j'\in A} \blambda_{\pi}(j') + 
	\sum_{j\not\in A}\blambda_{\pi}(j)= |A|\blambda_{\pi}(s) + 
	\sum_{i=1}^{k}\sum_{0\le j\le l_k}\blambda_{\pi}(s_k+j)\\
	&\le |A|\blambda_{\pi}(s) + \sum_{i=1}^{k} \sum_{0\le j\le  l_i} \frac{j+1}{T}
	\le |A|\blambda_{\pi}(s) + \sum_{i=1}^{k} \frac{(l_i+2)(l_i+1)}{2T}.
	\end{align*}
	Note that $S'=\sum_{i} l_i=\Theta(\sqrt{T})$, 
	\[
	\sum_{i=1}^{k} (l_i+2)(l_i+1)
	\le 6 \sum_{i=1}^{k} l_i^2 \le 6 \Big(\sum_{i=1}^{k} l_i\Big)^2 \le T/2
	\]
	for appropriately chosen $S'$.
	Thus,
	\begin{align*}
\blambda_{\pi}(s)\ge 
\frac{1}{|A|}\cdot  \bigg(1-\sum_{i=1}^{k} \frac{(l_k+2)(l_k+1)}{2T}\bigg) \ge  \frac{1}{2T}.
	\end{align*}
	We further notice that, for each state $i$ on an $R$-chain with source $s$, we have $\blambda_{\pi}(i) \ge \blambda_{\pi}(s)\ge 1/(2T)$, which completes the proof.
%
%	\begin{align*}
%	\forall s\in A:\quad \blambda_{\pi}(s) &= 
%	\sum_{j\in A}\blambda_{\pi}(j)\bP(i|j,\pi(j)) 
%	+\sum_{j\not\in A}\blambda_{\pi}(j)\bP(i|j,\pi(j))\\
%	& = \frac{|A|}{T}\cdot\blambda_{\pi}(s) + \sum_{j\not\in A}\blambda_{\pi}(j)\bP(i|j,\pi(j))
%	\ge \sum_{j\in A}\blambda_{\pi}(j)\bP(i|j,\pi(j)) . 
%	%\ge \frac{1-\sum_{i=1}^k l_i(l_i+1)/(2T) }{T} \ge \frac{1}{2T}-\frac{\sqrt{T}}{2T^2}.
%	\end{align*}
	%Note that for $s\in A$ and $j\not\in A$, $j$ has a non-zero transition probability to $s$ only when $j$ is the end of some $R$-chain.
	
	%We then immediately have 
	%\[
	%\blambda_{\pi}(s_i) \ge \frac{T-\sqrt{T}}{2T^2}-\frac{(T-\sqrt{T})\sqrt{T}}{2T^3} \ge \frac{1}{3T}
	%\]
	%for sufficiently large $T$.
	%
	%For a state $i$, suppose $\pi(i-1) = B$ and
	%\[
	%\lambda_{\pi}(i) = \sum_{j}\lambda_{\pi}(j) P(i|j, \pi(j)) 
	%< 1/(3T).
	%\]
	%Then it must be the case that $\sum_{\pi(i'-1)=R}\lambda_{\pi}(i')>2/(3T)$.
	%
	%
	%We observe that $\lambda_{\pi} = P_{\pi}^{\sqrt{T}} \lambda_\pi$.
	%
	%
	%%
	%For each policy $\pi$, we can decompose it into pieces, where each piece plays only $R$ actions and ends at a action $B$.
	%We denote policy $\pi=(b_1, b_2, \ldots, b_j)$ where contains the number of $R$ actions in each trunk.
	%Then the first $b_1-1$ rows of $\pi$ contain only a single $1$, follows by a $1/T$ row; then the $b_1+1$ to $b_1+b_2$ rows contain only a single $1$ again ...
	%For such a matrix, we can verify that the invariant distribution is 
	%\begin{align*}
	%\lambda_{\pi}
	% = \mathrm{normalize}\Big([
	% (1,2,\ldots, b_1, b_1+1), (1,2,\ldots, b_2-1), 1, \ldots, (1,2,\ldots, b_j-1), 1
	% ]\Big)
	%\end{align*}
	%Therefore, 
	%\[
	%\max_{s} \lambda_{\pi}(s) \le 
	%\max_{i}\frac{b_i}{T^2/j + \sum_{z}b_z^2}
	%\le \max_i\min\Big(\frac{jb_i}{T^2}, \frac{1}{b_i}\Big).
	%\]
	%And
	%\[
	%\min_{s} \lambda_{\pi}(s) \ge 2/[T(T-1)]
	%\]
	%Firstly, we notice that $\lambda_{\pi}(1) \le 1/T$.
	%This is because no other states has probability greater than $1/T$ transit to this state.
	%Because so, it must be the case that $\lambda_{\pi}(2) \le 1/T$. 
	%
	%Notice that for $P_{\pi}^\top$, each row can only contains a single $1$ but can contain multiple $1/T$s.
	%Let $r$ be the $i$th row of $P_{\pi}^\top$.
	%So $r(i-1)$ is either $1/T$ or $1$.
	%Suppose $\lambda_{\pi}(i)> C/T$ for some large constant $C$.
	%Then, if $r(i-1) = 1/T$
	%\[
	%\lambda_\pi(i) = r^\top \lambda_\pi \le  C/T / T +  1/T \le C/T,
	%\]
	%a contradiction.
	%It must be the case that $r(i-1) = 1$.
\end{proof}


Note that the flux ratio and ergodicity ratio can be arbitrarily close, as $\gamma\to1$. It can be seen that 
$
\lim_{\gamma \rightarrow 1}(1-\gamma)\bff^{\pi} =\blambda^\pi. 
$
Thus we have 
$
\lim_{\gamma \rightarrow 1}\delta_{\max}/\delta_{\min} = c_{\max}/c_{\min} = \Theta(\sqrt{T}). 
$



\paragraph{Proof of Theorem \ref{thm:pi-hard}.}
\begin{proof}
	We apply policy iteration (PI) to the MDP instance constructed above. Let the initial policy be $\pi^0$, which is to always choose action $U$.
	We will show that the PI improves the policy by changing at most one action at a time. 
	Let $\pi^{(i)}$ denote the policy which chooses $U$ at states  $1,2,\ldots,(T-i-1), T$  and chooses $R$ at states $T-i,\ldots,T-1$.
	It suffices to show that the PI improves the policy according to the sequence
	\[
	\pi^{(0)} \rightarrow \pi^{(1)} \rightarrow \pi^{(2)}\ldots \rightarrow   \pi^{\Theta(S')},
	\]
	thus the number of iterations needed is $\Theta(S')$, which is proportional to the flux ratio.
	
	We prove this by induction.
	Assuming that the current policy is $\pi^{(i-1)}$, we consider the next policy generated by PI.
	Let us analyze its value function $\bv^{\pi^{(i-1)}}$, and we let $\wb{v}^{(i-1)} = T^{-1}\sum_{s}\bv^{\pi^{(i-1)}}(s)$.
	By the Bellman equation for a fixed policy, we have
	\begin{align*}
	\bv^{\pi^{(i-1)}}(T) = r_T + \gamma \wb{v}^{(i-1)},&\quad
	\bv^{\pi^{(i-1)}}(T-j) = \gamma^j(r_T + \gamma \wb{v}^{(i-1)}) \quad\text{for } 1\le j \le i-1 \quad 
	\text{and} \quad \\
	\bv^{\pi^{(i-1)}}(T-j) &=  \gamma \wb{v}^{(i-1)}\quad \text{for}\quad  j\ge i.
	\end{align*}
	By solving the above equations, we obtain % can solve $\wb{\bv}^{(i-1)}$ as
	\[
	\wb{v}^{(i-1)} = 
	\frac{r_T (1 - \gamma ^i)}{T(1-\gamma)^2 - \gamma + i\gamma(1  - \gamma) + \gamma^{i+1}}.
	%\frac{r_T \cdot\frac{1-\gamma^{i}}{1-\gamma}}{
	%	T(1-\gamma) + i\gamma - \frac{1-\gamma^{i}}{1-\gamma}\cdot \gamma.
	%}
	\]
	Next we consider the policy improvement step using $\bv^{\pi^{(i-1)}}$. Denote $\bQ$ as the Q-function of $\pi^{(i-1)}$.
	\begin{enumerate}
	\item Consider states $T-j$ such that $1\le j\le i-1$, the policy improvement step compares the following two values:
	\begin{align*}
	\bQ(T-j, R) = \gamma^{j} (r_T + \gamma \wb{v}^{(i-1)}) 
	\quad \text{and} \quad 
	\bQ(T-j, U) = \gamma \wb{v}^{(i-1)}.
	\end{align*}
	Therefore as long as $\bQ(T-j, R) > \bQ(T-j, U)$ then the action will not be changed.
	For this to happen, we can pick $\gamma = 1-1/\beta$ for $\beta=\Omega(T)$.
	Then by using a Taylor expansion analysis we obtain $\wb{v}^{(i-1)} = \Theta(i\cdot r_T\cdot \beta/T)$ and $1-\gamma^j = \Theta(j/\beta)$.
	Thus $\bQ(T-j, R) = r_T + \gamma \wb{v}^{(i-1)} - O(ij/T\cdot r_T)$.
	Notice that $ij/T<1$ by our construction. Therefore as long as $r_T >0$ we have $\bQ(T-j, R) \ge \bQ(T-j, U)$.
	Hence, the $R$ action at these states will not be changed after one policy iteration. 
	\item
	Consider states $T-j$ such that $i \le j\le S'$, we have 
	\[
	\bQ(T-j, U) = \gamma \wb{v}^{(i-1)} >
	\bQ(T-j, R) = \gamma^2 \wb{v}^{(i-1)}.
	\]
	Thus, the optimal action at these states is still to choose $U$ over $R$. 
	\item Since the current policy is not optimal, the policy iteration will generate a different policy. Therefore the only action that can be changed is the one at state $T-i$.
	Indeed, we have
	\[\bQ(T-i, R) = r_T + \gamma \wb{v}^{(i-1)} - O(i^2/T\cdot r_T) \ge \bQ(T-i, U) = \gamma \wb{v}^{(i-1)}.
	\]
	\end{enumerate}
	Now we have verified that the next policy generated by the PI r is exactly $\pi^{(i)}$. By induction, we have shown that the PI will generate a sequence of policies where only one action is changed per policy evaluation.
	
	Finally we show that the policy iteration needs $\Theta(S')$ steps to find a sufficiently accurate solution. 
	Let  $i \le S'/4$.
	We would like to compare
	$\bv^{\pi^{(i)}}$ with 	$\bv^{\pi^{(S')}}$ as  we have, by monotonicity of PI,
	\[
	\bv^{\pi^{(S')}} - \bv^{\pi^{(i)}}
	\le \bv^{\pi^{*}} - \bv^{\pi^{(i)}}.
	\]
	Consider the state $T$. %for $j\le i-1$.
	We have
	\begin{align*}
	\bv^{\pi^{(i)}}(T)
	&=r_T + \gamma \wb{v}^{(i)}
	 %- O(i/T\cdot r_T)
	 %= r_T + \gamma \Theta(i\cdot r_T)\\
	 \le r_T + \gamma \Theta(i\cdot r_T\cdot \beta/T)
	 \le r_T + \Theta(1/4\cdot\gamma S' \cdot r_T\cdot \beta/T)
	\end{align*}
	and
	$
	\bv^{\pi^{(S')}}(T)
	=r_T + \gamma \Theta(S'\cdot r_T\cdot \beta/T)
	%\ge r_T + \Theta(3/4\cdot\gamma  S'\cdot r_T)
	$
	as long as $T$ is sufficiently large.
	Therefore,
	\[
	\bv^{\pi^{(S')}}(T-1) - \bv^{\pi^{(i)}}(T-1)
	\ge \Theta(1/2\cdot \gamma S'\cdot r_T\cdot \beta/T) \gg r_T.
	\]
	%\[
	%\bDelta(i)=  \gamma^{j}\Big(\wb{\bv}^{(i-1)}(T-j) - \wb{\bv}^{(\Theta(\sqrt{T}))}(T-j)\Big)
	%= \Theta\Big((1-j/T)\cdot \br_T\Big).
	%\]
	%For $i=\Theta(\sqrt{T})$ and $j=\Theta(i)$, we still have $\bDelta(i)\ge \Omega(1)$.
	Thus, after $\Theta(S')=\Theta(\sqrt{T})$ steps, the resulting policy is not yet $0.1$-optimal provided $r_T= 1$.
\end{proof}

\subsection{Lower Bound for Strategy Iteration}

Next we extend the lower bound to strategy iteration (SI). Recall that each iteration of SI requires solving a new MDP instance by using the policy iteration. %Note that each strategy iteration requires solving an MDP instance using policy iteration. 
Thus the total number of policy evaluations needed is quadratic in the flux ratio. In what follow we provide a matching lower bound.

\begin{theorem}\label{lowerbound}
	Consider the strategy iteration of the form:
	Initialize with some strategy $
	\sigma^{(0)}:=[\pi_{\min}^{(0)}, \pi_{\max}^{(0)}]$ and conduct the following at the $i$-th iteration:
	\begin{enumerate}
		\item[I.] Obtain the optimal max-player strategy $\pi_{\max}^{(i)}$ against $\pi_{\min}^{(i-1)}$ using policy iteration that is initiated with $[\pi_{\min}^{(i-1)}, \pi_{\max}^{(i-1)}]$;
		%\mw{si? typos?}
		\item[II.] Compute the new min-player strategy $\pi_{\min}^{(i)}$ as the greedy strategy of $\bv^{\sigma^{(i-1)}}$ for $\sigma^{(i-1)} = [\pi_{\min}^{(i-1)}, \pi_{\max}^{(i)}]$.
	\end{enumerate}
	Then there exists a 2TBSG instance with flux ratio $\delta_{\max}/\delta_{\min}$, and an initial strategy $\sigma^{(0)}$, such that the above 
	SI requires $\Omega(\delta^2_{\max}/\delta^2_{\min})$ policy evaluations to obtain an $0.1$-optimal policy.
\end{theorem}
\begin{figure}[htb!]
	\centering
	\includegraphics[width=0.8\textwidth]{hard_game.png}
	\caption{The hard instance (HI2) for strategy iteration.\label{fig:hcgame}}
\end{figure}
\paragraph{Hard instance of 2TBSG (HI2)}
Let there be five sets of states: $T$ dummy states, $S':=\Theta(\sqrt{T})$ min-player states, and $S'+1$ max-player states, $S_b:=\Theta(\sqrt{T})$ min-player boosting states,  $S_b':=\Theta(\sqrt{T})$ max-player boosting states  (Figure \ref{fig:hcgame}).
%The min-player states and the dummy states (in total $\Theta(T)$ many) form a similar structure as the policy iteration case.

The dummy states are also controlled by the min player but there is only one possible action at these states.

We denote the min-player states as $s_{m_1}, s_{m_2}, \ldots, s_{m_{S'}}$.
For each min player state, it has two actions.
The $U$ (uniform) action  transitions the state to every other state with a equal probability, with reward $0$.
The $R$ (right) action transitions $s_{m_{i}}$ to the next state $s_{m_{i-1}}$ and has a reward $r_{\delta}\ge 0$ (to be determined).

%For each min-player state, there is a max-player state attached to it, which we denote as $s_{m_1}', s_{m_2}', \ldots, s_{m_{S'}}'$.
%There is only one action for each $s_{m_i}'$ and we denote the reward of these actions as $r_{i}\ge 0$ (to be determined).

There is a goal state $s_g$.
From the min-player states to the goal state, there is a sequence of $S_b$ min-player boosting states,
$s_{b_1}, s_{b_2}, \ldots, s_{b_{S_b}}$.
These states has only one action $R$ and are chained together: $R$ transitions $s_{b_{S_b}}$ to $s_{b_{S_b-1}}$, $s_{b_{S_b-1}}$ to $s_{b_{S_b-2}}$, ..., $s_{b_{1}}$ to
$s_g$.
No reward is given to these actions.
The $R$ action transitions $s_{m_{1}}$ to $s_{b_{S_b}}$ with reward $r_{\delta}$.

$s_g$ has only one action which has a reward $-r_g$ (to be determined) and transitions to another state uniformly at random.

There is a sequence of max-player states $s_{M_1}, s_{M_2}, \ldots, s_{M_{S'}}$.
These states have two actions, one action $U$ transitions to another state uniformly at random, with reward $0$; one action $R$ transitions the state $s_{M_i}$ to $s_{M_{i-1}}$, with reward $-r_{\delta}'\le 0$ (to be determined).

The switching state $s_{*}$ has $S'$ actions which we denote as $a_1, a_2, \ldots, a_{S'}$.
The action $a_i$ will transition the state to state $s_{m_i}$ with reward $r_i$ (to be determined).

From the $s_{M_1}$ to the state $s_*$, there is a sequence of $S_b'$ max-player boosting states,
$s_{B_1}, s_{B_2}, \ldots, s_{B_{S'_b}}$. 
These states have only one action $R$ and are chained together: $R$ transitions $s_{B_{S_b'}}$ to $s_{B_{S_b'-1}}$, $s_{B_{S_b'-1}}$ to $s_{B_{S_b'-2}}$, ..., $s_{B_{1}}$ to
$s_*$.

The $R$ action transitions the state $s_{M_{1}}$ to the state $s_{B_1}$ with reward $-r_{\delta}'$.


Initially, the min-player policy $\pi_{\min}^{(0)}$ and the max-player policy $\pi_{\max}^{(0)}$ play action $U$ at every state except $s_*$;
$\pi_{\max}^{(0)}(s_*) = a_{1}$.

\paragraph{High Level Intuition}
To begin our formal discussion of the hard instance, we first remark the high level intuition of the lower bound.

We construct the instance such that the min-player is somewhat decoupled from the max-player.
That said, starting from the min-player policy $\pi_{\min}^{(0)}$ that plays action $U$  at every state $s_{m_j}$, the algorithm changes only one action at an iteration.
For instance, at iteration $i\in[1, S']$, the min-player policy, $\pi^{(i)}_{\min}$, plays action $U$ at state $s_{m_j}$ for all $j\in [i+1, S']$ and plays action $R$ at state $s_{m_{j'}}$ for $j'\in [i]$. The number of $U$ actions decreases as the iteration number $i$ increases.

However, the max-player policy is largely affected by the current choice of the min-player.
We will show, by induction, that $\pi_{\max}^{(i-1)}$ plays action $a_{i-1}$ at the switching state $s_*$.
In the beginning of iteration $i$, the present min-player policy is still $\pi_{\min}^{(i-1)}$, which ``chains'' together states $s_{i-1}, s_{i-2}, \ldots, s_{1}, s_{b_{S_b}}, s_{b_{S_b-1}},$ $\ldots, s_g$ by action $R$.
%However, %the max-play policy $\pi_{\max}^{(i-1)}$ plays action $a_{i-1}$ at state $s_*$ (by induction hypothesis).
%This 
Hence, the action $a_{i-1}$ connects the switching state $s_*$ to $s_{i-1}$, which is  eventually connected to the goal state $s_g$ by the min-player policy.
Note that the goal state $s_g$ has a negative reward, therefore $a_{i-1}$ is highly sub-optimal against $\pi_{\min}^{(i-1)}$.
By appropriate choices of $r_1, r_2, \ldots, r_{S'}$, $r_{\delta}$, and $r_{g}$ we can guarantee that the next step of the algorithm would take the  max-player  policy $\pi_{\max}^{(i, 0)}$, which plays action $U$ at every max-player state $s_{M_j}$ and action $a_{i}$ at state $s_*$ (e.g., choose $r_1> r_2> r_3 >\ldots, r_{S'}$).
For the rest iterations of step I., the algorithm would take $\Theta(\sqrt{T})$ steps to improve the policy $\pi_{\max}^{(i, 0)}$ until it is approximately optimal against the present min-player policy. This is in analogous to the lower bound proof of PI (Theorem~\ref{thm:pi-hard}). But for all these improvement steps, the action at $s_*$ is $a_i$ without changing.

Since there are $\Theta(\sqrt{T})$ min-player states,
the overall number of policy evaluations would be $\Theta(T)$.
However, we will show that the flux ratio of the instance is $\Theta(\sqrt{T})$.
Thus we prove a quadratic lower bound of SI over the flux ratio.

\paragraph{Formal Analysis}
In this section, we prove Theorem~\ref{lowerbound} formally.
The ergodicity and flux ratio of the hard instance is presented in the next lemma.
\begin{lemma}
	\label{lemma:ergodicity-strat}
	For any strategy $\sigma$, let $\blambda_\sigma$ be the invariant distribution on the hard instance, HI2.
	Then for sufficiently large $T$, we have
	\[
	\Theta(1/T) \le \blambda_{\sigma} \le \Theta(\sqrt{T}) /T.
	\]
	%for some constants $c, C$.
\end{lemma}
The proof is similar to that of Lemma~\ref{lemma:ergodicity}.
For completeness, we put a proof in the appendix.
Now we are ready to show a lower bound for SI.
Note that $\gamma$ can be made arbitrarily close to $1$. 
By Lemma~\ref{ratio:limit}, the hard instance has a flux ratio $\Theta(\sqrt{T})$ provided $\gamma$ sufficiently close to $1$.

To prove Theorem~\ref{lowerbound}, we first introduce some more notations.
\begin{definition}
We denote the min-player strategy $\pi^{(i)}_{\min}$ as follows:
\[
\pi^{(i)}_{\min}(s_{m_j}) = R \quad\text{for} \quad 1
\le j\le i, \quad \text{and}\quad \pi^{(i)}_{\min}(s_{m_{j'}}) = U \quad\text{for }j'>i. 
\]	
We also denote max-player strategy $\pi^{(i,z)}_{\max}$
for $z\in [0,S']$ as follows
\[
\pi^{(i,z)}_{\max}(s_{M_j}) = R \quad\text{for} \quad 1
\le j\le z, \quad \text{and}\quad \pi^{(i, z)}_{\max}(s_{M_{j'}}) = U \quad\text{for}\quad j'>z
\]
and $\pi^{(i,z)}_{\max}(s_{*}) = a_i$ for all $z\in [0,S']$.
\end{definition}
In what follows, we let
\[
r_{\delta}, r_{\delta}' = \Theta(1/\sqrt{T}), \gamma = 1-1/\beta \text{ with } \beta=\Omega(T), \quad\text{and}\quad S_b, S_b'> S'=\Theta(\sqrt{T}).
\]
The exact conditions of setting these values will become clear in the reminder of the text.
We now show some approximated values of the above policies in the next lemma.
\begin{lemma}
	\label{lemma:vbar}
Let $\wb{v}[\sigma] = \be^{\top} \bv^{\sigma}$.
Let $T'=(T+2S'+S_b+S_b'+2)$.
Then, for every $i\in [S'], z\in [0, S']$,
\begin{align*}
(1-\gamma)T'\cdot\wb{v}\Big[\big(\pi^{(i)}_{\min}, \pi^{(i, z)}_{\max}\big)\Big]
&= -(2+i+z+S_b+S_b') r_g + (1+z+S_b') r_i + c\sqrt{T}\quad\text{and}\quad\\
(1-\gamma)T'\cdot\wb{v}\Big[\big( \pi^{(i)}_{\min}, \pi^{(i+1, z)}_{\max}\big)\Big]
&= -(i+S_b+1) r_g + (1+z+S_b') r_i + O(1).
\end{align*}
for some $c\le1$ can be made arbitrarily small by controlling the ratio $S_b'/\sqrt{T}$ and provided $\gamma$ sufficiently close to $1$.
\end{lemma}
\begin{proof}
\textbf{Part I.} We first consider strategy, $\sigma=\big(\pi^{(i)}_{\min}, \pi^{(i,z)}_{\max}\big)$.
For the sake of representation, let $\wb{v} = \wb{v}\Big[(\pi^{(i)}_{\min}, \pi^{(i)}_{\max})\Big]$ and $\bv=\bv^{\sigma}$.
We also denote
\[
\Gamma[z] := \sum_{j=0}^{z-1}\gamma^j= \frac{1-\gamma^{z}}{1-\gamma}
\quad\text{and}\quad
B[z] := \sum_{j=1}^{z}\Gamma[j]
= \frac{\gamma z- \Gamma[z]}{1-\gamma}.
\]
In order to compute $\wb{v}$, we list the values of each state.
\begin{enumerate}
\item Min-player: for each $j\in [i]$: $\bv(s_{m_j}) = \gamma^{j+S_b}(-r_g + \gamma \wb{v}) + \Gamma[j]\cdot r_\delta$;
\item  Min-player: for each $j\in [i+1, S']$: $\bv(s_{m_j}) =\gamma \wb{v}$;
\item  Min-player-boosting: for each $j\in [S_b]$: $\bv({s_{b_j}}) = \gamma^{j}(-r_g + \gamma \wb{v})$
\item Dummy: for each dummy state $s$: $\bv(s) = \gamma \wb{v}$;
\item Max-player: for the switching state $s_*$: $\bv(s_{*}) = r_i + \gamma^{i + S_b+1}\cdot (-r_g + \gamma \wb{v}) + \gamma\Gamma[i]\cdot r_{\delta}$;
\item Max-player: for each $j\in [z]$: 
$\bv(s_{M_j}) = \gamma^{j+S_b'}\cdot[r_i + \gamma^{i+S_b+1}\cdot(-r_g + \gamma \wb{v}) + \gamma\Gamma[i]\cdot r_\delta] - \Gamma[j]\cdot r_{\delta}'$;
\item Max-player: for each $j\in [z+1, S']$: 
$\bv(s_{M_j}) = \gamma \wb{v}$;
\item Max-player-boosting: for each $j\in [S_b']$: $\bv({s_{b_j}}) =  \gamma^{j} (r_i +\gamma^{
i + S_b+1} (-r_g + \gamma \wb{v}) + \gamma\Gamma[i]\cdot r_{\delta})$;
\item Goal: for state $s_g$: $\bv(s_g) = -r_g + \gamma\wb{v}$;
\end{enumerate}
To computer the average value $\wb{v}$, we take a sum of the values of each state, i.e.,
\[
\one^\top \bv = (T+2S'+S_b+S_b'+2)\cdot \wb{v}.
\]
For the sake of representation, we compute $(1-\gamma) \wb{v}$ under the limit of $\gamma\rightarrow 1$\footnote{Note this is without loss of generality since we can make $\gamma$ arbitrarily close to $1$.}.
In this case $\Gamma[z] \rightarrow z$, and $B[z]\rightarrow z(z-3)/2$.
Note that 
%all the terms of $\gamma \wb{v}$ in $\one^\top \bv$ can be collected as the following form
%\[
%\gamma\cdot (T+2S'+S_b+S_b'+2)\cdot \wb{v}.
%\]
%Therefore, we have
\begin{align}
\label{eqn:sum-v}
\underset{\textcircled{1}}{\underline{\one^\top \bv - \gamma\cdot (T+2S'+S_b+S_b'+2)\cdot \wb{v}}}
 = (T+2S'+S_b+S_b'+2)\cdot \wb{v} \cdot(1-\gamma).
\end{align}
To compute $(1-\gamma) \wb{v}$, it suffices to compute the left hand side of the above equation.
We further notice that under the limit of $\gamma\rightarrow 1$, all the terms contributed by $\gamma \wb{v}$ can be canceled exactly.
For the rest of the terms, we can compute
\begin{align*}
\textcircled{1} &= 
\underset{\text{from 1.-3.}}{\underline{i\cdot(-r_g) + (i-3)i/2\cdot r_\delta
+ S_b\cdot (-r_g)}} 
+ 
\underset{\text{from 5.}}{\underline{r_i + (-r_g) + i\cdot r_\delta}}
\\
&\qquad+
\underset{\text{from 6.}}{\underline{z\cdot r_i + z\cdot (-r_g) + zi\cdot r_\delta - z(z-3)/2\cdot r_{\delta}'}} + 
\underset{\text{from 8.-9.}}{\underline{S_b'\cdot r_i + S_b'\cdot (-r_g) + S_b'i\cdot r_\delta - r_g}}.
\end{align*}
Since $r_\delta, r_{\delta}'\in \Theta(1/\sqrt{T})$, we have $[(i-3)i/2+zi+S_b'i]\cdot r_{\delta} = O(\sqrt{T})$ and $(z-3)z/2\cdot r_{\delta}' = O(1)$.
Thus
\[
\textcircled{1} =
-(2+i+z+S_b+S_b') r_g + (1+z+S_b') r_i + c\sqrt{T}
\]
for some $c=\Theta(1)$.

\noindent\textbf{Part II.} 
Next we consider $\sigma=\big(\pi^{(i)}_{\min}, \pi^{(i+1, z)}_{\max}\big)$.
Similarly, we compute the values.
\begin{enumerate}
	\item Min-player: for each $j\in [i]$: $\bv(s_{m_j}) = \gamma^{j+S_b}(-r_g + \gamma \wb{v}) + \Gamma[j]\cdot r_\delta$;
	\item  Min-player: for each $j\in [i+1, S']$: $\bv(s_{m_j}) =\gamma \wb{v}$;
	\item  Min-player-boosting: for each $j\in [S_b]$: $\bv({s_{b_j}}) = \gamma^{j}(-r_g + \gamma \wb{v})$
	\item Dummy: for each dummy state $s$: $\bv(s) = \gamma \wb{v}$;
	\item Max-player: for the switching state $s_*$: $\bv(s_{*}) = r_i + \gamma^2\wb{v}$;
	\item Max-player: for each $j\in [z]$: 
	$\bv(s_{M_j}) = \gamma^{j+S_b'}\cdot(r_i + \gamma^2 \wb{v}) - \Gamma[j]\cdot r_{\delta}'$;
	\item Max-player: for each $j\in [z+1, S']$: 
	$\bv(s_{M_j}) = \gamma \wb{v}$;
	\item Max-player-boosting: for each $j\in [S_b']$: $\bv({s_{b_j}}) =  \gamma^{j} (r_i +\gamma^2\wb{v})$;
	\item Goal: for state $s_g$: $\bv(s_g) = -r_g + \gamma\wb{v}$;
\end{enumerate}
To compute $\wb{v}$, we consider  the same formula as in \eqref{eqn:sum-v}.
Now we have
\begin{align*}
\textcircled{1} &= 
\underset{\text{from 1.-3.}}{\underline{i\cdot(-r_g) + (i-3)i/2\cdot r_\delta
		+ S_b\cdot (-r_g)}} 
+
\underset{\text{from 5.-9.}}{\underline{r_i+z\cdot r_i - z(z-3)/2\cdot r_{\delta}'+ S_b'\cdot r_i - r_g}}.
\end{align*}
Again, since $r_\delta, r_{\delta}'\in \Theta(1/\sqrt{T})$, we have $[(i-3)i/2]\cdot r_{\delta} = O(1)$ and $(z-3)z/2\cdot r_{\delta}' = O(1)$.
Thus
\[
\textcircled{1} =
-(i+S_b+1) r_g + (1+z+S_b') r_i + O(1).
\]
%
%Since $\gamma=1-1/\Omega(T)$, we can let 
%$\gamma^{\Theta(\sqrt{T})}$ to be arbitrarily close to $1$ (taking $T$ to be sufficiently large). 
%
%For what follows, we let ``$\approx$'' denote an approximation up to factor $\gamma^{O(\sqrt{T})} = 1-O(1/\sqrt{T})$.
%Therefore, the value of each state $s_{b_j}$ 
%%has value 
%%in the range
%%$[-r_g + \gamma \wb{v}, \gamma^{\Theta(S_b)}(-r_g + \gamma \wb{v})]$ and 
%can be approximated by
%\[
%\bv^{\sigma}(s_{b_j}) = \gamma^{O(S_b)}(-r_g + \gamma \wb{v}) \approx -r_g + \gamma \wb{v}.
%\]
%Similarly, 
%for all $j\in [i]$,
%\[
%\bv^{\sigma}(s_{m_j})\approx j r_\delta'  -r_g + \gamma \wb{v},\quad \text{and}\quad \bv^{\sigma}(s_{m_j}')\approx j r_\delta' + r_{j'}-r_g + \gamma \wb{v}.
%%, \quad \text{and}\quad
%%\bv^{\sigma}(s_{M_j}) \approx r_\delta + r_i -r_g + \gamma \wb{v}.
%\]
%Therefore,
%for the values of $s_*$ and $s_{B_j}$, we have
%\[
%\bv^{\sigma}(s_{*})\approx \bv^{\sigma}(s_{B_j}) \approx r_i-r_g + \gamma \wb{v} + i r_{\delta}'.
%\]
%For each $z\in [S_b']$ such that $S_{M_z}$ is connected to the goal state $s_g$, we have
%\[
%\bv^{\sigma}(s_{M_j}) \approx ir_\delta'-zr_{\delta} + r_i -r_g + \gamma \wb{v}.
%\]
%For each $s$ that is not connected to goal state, we have,
%\[
%\bv^{\sigma}(s) = \gamma \wb{v} \quad\text{and}
%\quad \bv^{\sigma}(s_g) = -r_g + \gamma \wb{v}.
%\]
%Overall, we obtain
%\begin{align*}
%(T+3S' + 1 +S_b +S_b')\gamma \wb{v}
%&+ \Theta(S_b)\cdot (-r_g)
%+ \Theta(S_b')\cdot (-r_g + r_i) + \Theta({T})(r_\delta' - r_\delta)
%+ \sum_{j}r_{j}\\
%&= (T+3S' + 1 +S_b +S_b') \wb{v}.
%\end{align*}
%Since $(1-\gamma)T = \Theta(1)$, $\Theta(\sqrt{T})(r_\delta' - r_\delta)= O(1)$ and 
%$\sum_{j}r_j = \Theta(\sqrt{T})$, we have
%\[
%\wb{v}\Big[(\pi^{(i)}_{\min}, \pi^{(i)}_{\max})\Big] = \Theta\Big[-(S_b+S_b')r_g + S_b' r_i + \sum_{j}r_j\Big].
%\]
%
%By a similar argument, we have
%\[
%\wb{v}\Big[(\pi^{(i)}_{\min}, \pi^{(i+1, z)}_{\max})\Big]
%= \Theta\Big[-S_br_g + S_b' r_{i+1} + \sum_{j}r_j\Big].
%\]
\end{proof}
\begin{remark}
For some choices of  $S_b =\Theta(S_b') = \Theta(\sqrt{T})$ and $r_i = \Theta(r_g) = \Theta(1)$, we can have
\[
\wb{v}\Big[(\pi^{(i)}_{\min}, \pi^{(i, z)}_{\max})\Big] 
= -\Theta(\sqrt{T}) <0 \quad\text{and}
\quad \wb{v}\Big[(\pi^{(i)}_{\min}, \pi^{(i+1, z)}_{\max})\Big] = \Theta(\sqrt{T}) >0.
\] 
\end{remark}

To prove Theorem \ref{lowerbound},
it suffices to show,  by assigning appropriate values to $r_1, r_2, \ldots, r_{S'}, r_{\delta}, r_{\delta}', r_g$, the strategy iteration follows the following path.
\paragraph{Algorithm Path}
\begin{enumerate}
	\item The initial strategy is $(\pi_{\min}^{(0)},\pi_{\max}^{(0)})$;
	\item At iteration $i$,  the Step I is a PI for a fixed min-player strategy. The first iteration of this PI always initializes the max-player policy to be $\pi_{\max}^{(i+1,0)}$, if this is not this policy;
	\item  Step I of the algorithm takes $\Theta(\sqrt{T})$ policy evaluations to complete;
	% \mw{check this}
	% which satisfies
	%\[
	%\pi_{\max}^{(i,0)}(s_{M_1}) = U \quad\text{and}\quad 
	%\pi_{\max}^{(i,0)}(s_{*}) = a_{i};
	%\]
	%in  the $z$-th inner loop for $z\ge 0$, the algorithm takes the max-player policy to $\pi^{(i,z)}_{\max}$;
	%it ends after $Z_i=\Theta(\sqrt{T})$ iterations and assigns
	%$\pi^{(i)}_{\max} \gets \pi^{(i,Z_i)}_{\max}$;
	%to obtain an (approximate-)optimal strategy, $\pi_{\max}^{(i)}$, against the min-player strategy $\pi_{\min}^{(i-1)}$;
	%Moreover, the $\pi_{\max}^{(i)}$
	%plays action $R$ on states 
	%\[
	%s_{M_1}, s_{M_{2}}, \ldots,
	%s_{M_{Z_i}}
	%\]
	%for $Z_i = \Theta(\sqrt{T})$ and plays action $U$ on other states (except $s_*$);
	\item Step II of the iteration $i$ updates the min-player policy to $\pi_{\min}^{(i)}$;
	\item The algorithm takes $\Theta(\sqrt{T})$ iterations to finish.
	%that satisfies
	%\[
	%\forall 1\le j\le i:\quad \pi_{\max}^{(i)}(s_{m_{i}}) = R\quad\text{and}\quad
	%\forall i< j' \le S':\quad  \pi_{\max}^{(i)}(s_{m_{j'}}) = U,
	%\]
	%regardless of the current max-player strategy.
\end{enumerate}
In order to show that the algorithm always follow the above path, we verify the following key steps.
\begin{lemma}
\label{lem:si-improve1}
Suppose now the current status of the algorithm is at iteration $i\ge 0$ and step I.
If the current strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i, z)})$ for any $z\in [S']$, then the next strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, 0)})$, provided appropriately chosen values for $\{r_i\}_{i\in[S']}\cup\{r_\delta,r_\delta', r_g\}$.
\end{lemma}
\begin{proof}
	To prove this lemma, we will compare the action values at each max-player state and show that the actions of $\pi_{\max}^{(i+1, 0)}$ will be picked.
	
	
	Denote $\wb{v} = \wb{v}(\pi_{\max}^{(i)}, \pi_{\max}^{(i, z)})$
	and $\bQ = \bQ^{[\pi_{\max}^{(i)}, \pi_{\max}^{(i, z)}]} \in \RR^{\cS\times\cA}$ as the action value function.
	
	We first consider the switching state $s_*$.
	Recall that $s_*$ has $S'$ actions $a_1, a_2, \ldots, a_{S'}$.
	For each $j\in [i]$, we have
	\[
	\bQ(s_*, a_{j}) = r_j + \gamma^{i+S_b + 1}\cdot(-r_g + \gamma \wb{v}) + \gamma \Gamma[i]\cdot r_{\delta}.
	\]
	For each $j'\in [i+1, S']$, we have
	\[
	\bQ(s_*, a_{j'}) = r_{j'} +  \gamma^2 \wb{v}.
	\]
	Since we are choosing $r_1\ge r_2\ge \ldots r_{S'}$, action $a_{i+1}$ is more preferable to $a_{i+2}, a_{i+3}, \ldots, a_{S'}$.
	It remains to compare $\bQ(s_*, a_{i+1})$ with $\bQ(s_*, a_{j})$ for $j\in [i]$. Recall that $\gamma =1-1/\beta = 1-O(1/T)$, and $\wb{v} = -\Theta(\beta/T\cdot \sqrt{T})$ (by Lemma~\ref{lemma:vbar}).
	We thus have
	\[
	|\gamma^{i+S_b+1} (-r_g + \gamma \wb{v}) - (-r_g+\gamma^2 \wb{v})| = \Theta(1)
	\]
	which can be made arbitrarily small by controlling the ratio of $S_b/\sqrt{T}$.
	Note that $\gamma \Gamma[i] \cdot r_{\delta} = O(1)$ and can be made arbitrarily small by controlling the ratio of $S_b/\sqrt{T}$ as well.
	Therefore, for $j\in[i]$
	\[
	\bQ(s_*, a_{j}) \le r_j - r_g +  \gamma^2 \wb{v} + c
	\]
	for some constant $c$ that can be made arbitrarily small.
	Therefore, $a_{i+1}$ is preferable to $a_{j}$ as long as $r_{i+1}\ge r_{j} - r_g + c$, which can be guaranteed by choosing these values appropriately.
	
	Next, we show that for the state $s_{M_j}$ with $j\in [z]$, action $U$ is preferable.
	We can compute their action values as follows.
	\[
		\bQ(s_{M_j}, U) = \gamma \wb{v} \quad\text{and}\quad 
		\bQ(s_{M_j}, R) =  \gamma^{j+S_b'}\cdot[r_i + \gamma^{i+S_b+1}\cdot(-r_g + \gamma \wb{v}) + \gamma\Gamma[i]\cdot r_\delta] - \Gamma[j]\cdot r_{\delta}'.
	\]
	With a similar Taylor expansion argument as that for $s_*$, we have
	\[
	|\bQ(s_{M_j}, R) - (r_i - r_g +\gamma \wb{v})| = \Theta(1) 
	\]
	which can be arbitrarily small by controlling the ratios, $S_b/\sqrt{T}$ and $S_b'/\sqrt{T}$.
	Therefore, as long as $r_i-r_g+c\le 0$ for some small constant $c>0$, then
	$Q(s_{M_j}, R)<Q(s_{M_j}, U)$ and thus action $U$ is preferable.
	
	We now consider state $s_{M_{j'}}$ for $j'\in[z+1, S']$. We can compute their action values as follows.
	\[
	\bQ(s_{M_{j'}}, U) = \gamma \wb{v} \quad\text{and}\quad 
	\bQ(s_{M_{j'}}, R) = -r_{\delta}' + \gamma^2 \wb{v}.
	\]
	Since $|\gamma^2\wb{v} -\gamma \wb{v}| = O(1/\sqrt{T})$, and $r_{\delta}'= \Theta(1/\sqrt{T})$, we can make sure that
	\[
	\bQ(s_{M_{j'}}, U) > \bQ(s_{M_{j'}}, R) 
	\]
	by choosing $r_{\delta}'$ appropriately.
	This completes the proof.
\end{proof}
\begin{lemma}
	\label{lem:si-improve2}
	Suppose now the current status of the algorithm is at iteration $i\ge 0$ and step I.
	If the current strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)})$ for any $z\in [S'-1]$, then the next strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z+1)})$, provided appropriately chosen values for $\{r_i\}_{i\in[S']}\cup\{r_\delta,r_\delta', r_g\}$.
\end{lemma}
\begin{proof}
The proof is in a similar structure as that of Lemma~\ref{lem:si-improve1}.
We will compare action values at different states of the max-player.

	Denote $\wb{v} = \wb{v}(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)})$
and $\bQ = \bQ^{[\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)}]} \in \RR^{\cS\times\cA}$ as the action value function.

We first consider the state $s_*$.
For each $j\in [i]$, we have
\[
\bQ(s_*, a_{j}) = r_j + \gamma^{i+S_b + 1}\cdot(-r_g + \gamma \wb{v}) + \gamma \Gamma[i]\cdot r_{\delta}.
\]
For each $j'\in [i+1, S']$, we have
\[
\bQ(s_*, a_{j'}) = r_{j'} +  \gamma^2 \wb{v}.
\]
Since we are choosing $r_1\ge r_2\ge \ldots r_{S'}$, action $a_{i+1}$ is more preferable to $a_{i+2}, a_{i+3}, \ldots, a_{S'}$.
It remains to compare $\bQ(s_*, a_{i+1})$ with $\bQ(s_*, a_{j})$ for $j\in [i]$. Recall that $\gamma =1-1/\beta = 1-O(1/T)$, and $\wb{v} = \Theta(\beta/T\cdot \sqrt{T})$ (by Lemma~\ref{lemma:vbar}).
We thus have
\[
|\gamma^{i+S_b+1} (-r_g + \gamma \wb{v}) - (-r_g+\gamma^2 \wb{v})| = \Theta(1)
\]
which can be made arbitrarily small by controlling the ratio of $S_b/\sqrt{T}$.
Note that $\gamma \Gamma[i] \cdot r_{\delta} = O(1)$ and can be made arbitrarily small by controlling the ratio of $S_b/\sqrt{T}$ as well.
Therefore, for $j\in[i]$
\[
\bQ(s_*, a_{j}) \le r_j - r_g +  \gamma^2 \wb{v} + c
\]
for some constant $c$ that can be made arbitrarily small.
Therefore, $a_{i+1}$ is preferable to $a_{j}$ as long as $r_{i+1}\ge r_{j} - r_g + c$, which can be guaranteed by choosing these values appropriately.

Next, we show that for the state $s_{M_j}$ with $j\in [z+1]$, action $R$ is preferable.
We can compute their action values as follows.
\[
\bQ(s_{M_j}, U) = \gamma \wb{v} \quad\text{and}\quad 
\bQ(s_{M_j}, R) =  \gamma^{j+S_b'}\cdot(r_i + \gamma^2 \wb{v}) - \Gamma[j]\cdot r_{\delta}'.
\]
With a similar Taylor expansion argument as that for $s_*$, we have
\[
|\bQ(s_{M_j}, R) - (r_i +\gamma \wb{v})| = \Theta(1) 
\]
which can be arbitrarily small by controlling the ratio, $S_b'/\sqrt{T}$.
Therefore, as long as $r_i - c > 0$ for some small constant $c>0$, then
$Q(s_{M_j}, U)<Q(s_{M_j}, R)$ and thus action $R$ is preferable.

We now consider state $s_{M_{j'}}$ for $j'\in[z+2, S']$. We can compute their action values as follows.
\[
\bQ(s_{M_{j'}}, U) = \gamma \wb{v} \quad\text{and}\quad 
\bQ(s_{M_{j'}}, R) = -r_{\delta}' + \gamma^2 \wb{v}.
\]
Since $|\gamma^2\wb{v} -\gamma \wb{v}| = O(1/\sqrt{T})$, and $r_{\delta}'= \Theta(1/\sqrt{T})$, we can make sure that
\[
\bQ(s_{M_{j'}}, U) > \bQ(s_{M_{j'}}, R) 
\]
by choosing $r_{\delta}'$ appropriately.
This completes the proof.
\end{proof}
\begin{lemma}
	\label{lem:si-improve3}
	Suppose now the current status of the algorithm is at iteration $i\ge 0$ and step II.
	If the current strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)})$ for any $z\in [S']$, then the next strategy is $(\pi_{\max}^{(i+1)}, \pi_{\max}^{(i+1, z)})$, provided appropriately chosen values for $\{r_i\}_{i\in[S']}\cup\{r_\delta,r_\delta', r_g\}$.
\end{lemma}
\begin{proof}
To prove this lemma, we will compare the action values for the min-player.

Denote again $\wb{v} = \wb{v}(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)})$
and $\bQ = \bQ^{[\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)}]} \in \RR^{\cS\times\cA}$ as the action value function.

For each $j\in[i+1]$, we have
\[
\bQ(s_{m_j}, U) = \gamma \wb{v} \quad \text{and}\quad 
\bQ(s_{m_j}, R) = \gamma^{i+S_b}\cdot(-r_g + \gamma \wb{v}) + \Gamma[i]\cdot r_{\delta}.
\]
By a similar Taylor expansion argument, we have
\[
Q(s_{m_j}, R) \le -r_g + \gamma \wb{v} + c
\]
for some constant $c> 0$ that can be made arbitrarily small.
Therefore, as long as $-r_g+c<0$, action $R$ is preferable (note that the min-player prefers action with smaller action value).

For each $j'\in[i+2, S']$, we have
\[
\bQ(s_{M_{j'}}, U) = \gamma \wb{v} \quad\text{and}\quad 
\bQ(s_{M_{j'}}, R) = r_{\delta} + \gamma^2 \wb{v}.
\]
Since $|\gamma^2\wb{v} -\gamma \wb{v}| = O(1/\sqrt{T})$, and $r_{\delta}= \Theta(1/\sqrt{T})$, we can make sure that
\[
\bQ(s_{M_{j'}}, U) < \bQ(s_{M_{j'}}, R) 
\]
by choosing $r_{\delta}$ appropriately.
This completes the proof.
\end{proof}


\paragraph{Proof of Theorem \ref{lowerbound}}
%\mw{This proof is very informal}
\begin{proof}%[Proof Sketch]
By Lemma~\ref{lem:si-improve1}, \ref{lem:si-improve2}, and \ref{lem:si-improve3}, we can verify that the algorithm 
follows the following path,
\begin{align*}
(\pi_{\min}^{(0)}, \pi_{\max}^{(0)})&\rightarrow(\pi_{\min}^{(0)}, \pi_{\max}^{(1,0)})\rightarrow(\pi_{\min}^{(0)}, \pi_{\max}^{(1,1)})\rightarrow(\pi_{\min}^{(0)}, \pi_{\max}^{(1,2)})\ldots\rightarrow(\pi_{\min}^{(0)}, \pi_{\max}^{(1, S')})\\
\rightarrow(\pi_{\min}^{(1)}, \pi_{\max}^{(1, S')})&\rightarrow(\pi_{\min}^{(1)}, \pi_{\max}^{(2,0)})\rightarrow(\pi_{\min}^{(1)}, \pi_{\max}^{(2,1)})\rightarrow(\pi_{\min}^{(1)}, \pi_{\max}^{(2,2)})\ldots\rightarrow(\pi_{\min}^{(1)}, \pi_{\max}^{(2, S')})\\
&\ldots\\
\rightarrow(\pi_{\min}^{(S'-1)}, \pi_{\max}^{(S'-1, S')})&\rightarrow(\pi_{\min}^{(S'-1)}, \pi_{\max}^{(S',0)})\rightarrow(\pi_{\min}^{(S'-1)}, \pi_{\max}^{(S',1)})\rightarrow\ldots\rightarrow(\pi_{\min}^{(S'-1)}, \pi_{\max}^{(S', S')}).
\end{align*}
Each policy improvement step takes one policy evaluation.
By a straightforward counting, the total number of policy evaluations is $(S'-1)S' = \Theta(T)$.
%
%We hereby fix an iteration number $i\ge 0$.
%\begin{enumerate}
%\item[T1:] Step II:
%\item[T2:] Step II: if the current strategy is $(\pi_{\max}^{(i)}, \pi_{\max}^{(i+1, z)})$
%\end{enumerate}
%
%At iteration $i$, we first show that at the beginning of Step I of the algorithm, the max-play policy switches from $\pi^{(i-1)}_{\max}$ to $\pi^{(i,0)}_{\max}$.
%It holds for $i=1$ automatically.
%Consider $i>1$.
%For state $s_*$, we have, for $j<i$
%\[
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i-1)}_{\max}]}
%(s_*, a_j) = \gamma(r_j + \Theta(j)r_{\delta}' + \gamma^{S_b+j+1}(-r_g + \gamma \wb{v}))
% = \gamma(r_j + \wb{v} + \Theta(S_b/T)\cdot\wb{v} - r_g)),
%\]
%where we use the fact that $\Theta(j)r_{\delta}' = O(1)$ and $\Theta(S_b/T)\cdot\wb{v} = \Theta(1)$, 
%and for $i\le j'\le S'$
%\[
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i-1)}_{\max}]}
%(s_*, a_{j'}) = \gamma(r_{j'} + \gamma^2\wb{v})
%= \gamma(r_{j'} + \wb{v} + o(1)).
%\]
%Therefore, as long as 
%\[
%r_{i} < r_{i-1} < r_{i} +  r_g- \Theta(S_b/T)\cdot\wb{v},
%\]
%the action of $s_*$ will be switched to $a_i$.
%It remains to show that the action in every $s_{M_j}$ will be switched to $U$.
%Indeed, $\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i-1)}_{\max}]}
%(s_{M_j}, U) = \gamma \wb{v} = \wb{v} - O(1/\sqrt{T})$ and 
%\begin{align*}
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i-1)}_{\max}]}
%(s_{M_j}, R) &= \gamma^{O(S_b+S_b')} \wb{v}
%+ \gamma^{O(S_b')} r_{i-1} - \gamma^{O(S_b + S_b')} r_{g} - O(\sqrt{T})r_{\delta} + O(\sqrt{T})r_{\delta}'\\
%&= \wb{v} + O(r_{i-1}- r_{g} + O(1)).
%\end{align*}
%Therefore, as long as $r_{g} \ge r_{i-1}+\Theta(1)$ and $r_\delta  =\Theta(1/\sqrt{T})$, the action $U$ will be chosen in the first iteration.
%
%
%Next it can be verify that, during the inner loop of Step I, each policy iteration changes one action at a time via a similar argument as the proof of Theorem~\ref{thm:pi-hard}.
%Therefore, after all $\Theta(\sqrt{T})$ inner policy iterations, we obtain a max-player policy $\pi_{\max}^{(i)}$.%:=\pi_{\max}^{(i, Z_i)}$.
%
%It remains to show that each iteration of SI updates exactly one action in the min-player policy (in Step II).
%Note that now $\wb{v}:=\wb{v}\Big[(\pi^{(i-1, z)}_{\min}, \pi^{(i)}_{\max})\Big] = \Theta(\sqrt{T}) > 0$.
%For each state $s_{m_j}$ with $j<i$, we can verify that 
%\[
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i)}_{\max}]}
%(s_{m_j}, R)
%= O(\sqrt{T})r_{\delta}' + \gamma^{O(S_b)} \wb{v}
%- \gamma^{O(S_b)} r_{g}
% = -r_g + \wb{v} + O(1)
%\]
%and 
%\[
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i)}_{\max}]}
%(s_{m_j}, U)
%= \gamma \wb{v}=   \wb{v} + o(1).
%\]
%Therefore $\pi^{(i)}_{\min}(s_{m_j}) =\pi^{(i-1)}_{\min}(s_{m_j}) = R$.
%By using an analogous argument, we see
%\[
%\pi^{(i)}_{\min}(s_{m_i}) =R.
%\]
%For each state $s_{m_{j'}}$ with ${j'} > i$, 
%we have
%\[
%\bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i)}_{\max}]}
%(s_{m_{j'}}, R)
%= r_\delta' + \gamma^2\wb{v} =  r_\delta' + \wb{v} + o(1) \ge \bQ^{[\pi^{(i-1)}_{\min}, \pi^{(i)}_{\max}]}(s_{m_{j'}}, U)
%= \gamma \wb{v} = \wb{v} + o(1)
%\]
%for appropriately chosen $r_\delta'$.
%This completes the proof.
\end{proof}
\begin{remark}
If Step I. of the SI does not compute an exact optimal max-player strategy but an approximate one, a similar lower bound still holds.
This is because in the above proof, the PI in step I. require $\Omega(\sqrt{T})$ steps to finish even for an approximate optimal max-player strategy.
\end{remark}




%
%
%
%
%
%We first verify that the the above claim holds for iteration $1$ and then show, by induction on the iteration number $i$, it holds for all iterations $i\in[S']$. 
%
%We set 
%\[
%0<r_{S'}<r_{S'-1}\ldots <r_{1}.
%\]
%In the beginning of the first iteration, 
%the max-player already plays $\pi_{\max}^{1,0}$, verifying 1.
%
%%the max-player plays $a_{1}$ at state $s_*$ and the min-player plays action $U$ at state $s_{m_S'}$.
%Since $\forall 1< j\le S':~ r_{j}< r_{1}$, the algorithm will not change the action at $s_*$.
%Since $\wb{v}[\pi^{(0)}_{\min}, \pi^{(1, 1)}_{\max}] > 0$,
%by a nearly identical argument of the proof in Theorem~\ref{thm:pi-hard}, step I. of the algorithm takes $Z_1 = \Theta(\sqrt{T})$ steps to obtain a policy $\pi^{(1, 1)}_{\max}, \pi^{(1, 2)}_{\max}, \ldots, \pi^{(1, Z_i)}_{\max}$.
%This verifies 2.
%
%Now, we consider the min-player.
%Although $\wb{v}[\pi^{(0)}_{\min}, \pi^{(1, Z_1)}_{\max}] > 0$, the actions at state $s_{m_j}$ for $j\le i-1$ will not be changed:
%\[
%\bQ^{[\pi^{(0)}_{\min}, \pi^{(1, Z_1)}_{\max}]}
%(s_j, R) \le S'r_{\delta}' +  \gamma^{S_b} \wb{v}[\pi^{(0)}_{\min}, \pi^{(1, Z_1)}_{\max}] \le \bQ^{[\pi^{(0)}_{\min}, \pi^{(1, Z_1)}_{\max}]}
%(s_j, U) = \gamma \wb{v}[\pi^{(0)}_{\min}, \pi^{(1, Z_1)}_{\max}]	
%\]
%by choosing $r_\delta', S_b, S_b'$ appropriately.
%What next is to take action $R$ at state $s_{m_i}$.
%%By a nearly identical argument of the proof in Theorem~\ref{thm:pi-hard}, step II. of the algorithm switches the action to $R$ at state $s_{m_{S'}}$ with other states un-touched.
%This verifies 3. 
%
%Now suppose the claim holds for iteration $1, 2, \ldots, i-1$.
%Consider iteration $i>1$.
%At step I. of $i$, the policy iteration is initialized with 
%$\sigma^{(i-1)} = [\pi^{(i-1)}_{\min}, \pi_{\max}^{(i-1)}]$
%with 
%$\pi_{\max}^{(i-1)}
%(s_{*}) = 
%a_{S'-i+2}.
%$
%However, 
%\begin{align*}
%\pi_{\min}^{(i-1)}(s_{m_{S'-i+1}})
%&= U \quad\text{and}\quad \\
%\pi_{\min}^{(i-1)}(s_{m_{S'-i+2}})
%&= \pi_{\min}^{(i-1)}(s_{m_{S'-i+3}})
%=
%\pi_{\min}^{(i-1)}(s_{m_{S'-i+4}})
%\ldots 
%=\pi_{\min}^{(i-1)}(s_{m_{S'}})
%= R.
%\end{align*}
%Let
%\[
%\wb{v}^{(i-1)}) = \sum_s \bv^{\sigma^{(i-1)}}(s)\cdot\frac{1}{T+2S'+1}.
%\]
%Solving the Bellman equation, we obtain
%
%
%
%Therefore,
%\begin{align*}
%\bQ^{\sigma^{(i-1)}}(s_{*}, a_{S'-i+2})
%&= \gamma\cdot r_{S'-i+2}
%+ \gamma^{i+1}\cdot(-r_g + \gamma\cdot \wb{v}^{(i-1)})
%\quad\text{and}\\
%\bQ^{\sigma^{(i-1)}}(s_{*}, a_{S'-i+1})
%&= \gamma\cdot r_{S'-i+2}
%+ \gamma^3 \cdot\wb{v}^{(i-1)}
%\end{align*}
%where
%
%
%To the begin the proof, we first explain the intuition.
%We set $1/2\le r_1 < r_2 < r_3 \ldots < r_g$. 
%Consider the initial strategy $\sigma^{(0)}$ which plays the action $U$ at every state except for state $s_*$. For $s_*$, it plays action $a_{\sqrt{T}}$. 
%According to SI, the min-player strategy will improve according to: start with $U$ at every state, the next strategy picks $R$ starting at the second last state, the third strategy picks $R$ beginning at the third last state, and so on.
%In the mean time, the max-player strategies are updated as the best responses to the min strategies, i.e., starting with picking $r_7$, the next strategy is to always move up and pick $r_6$, and so on.
%
%
%Consider the min-player. It requires to improve for at least $\Theta(\sqrt{T})$ times for an arbitrary choice of $r_g\ge 1/2$ to be sufficiently close-to-optimal (similar to Theorem~\ref{thm:pi-hard}).
%
%Consider the inner policy iteration for the max-player. 
%Initially, since the min-player plays action $U$ at state $s_{m_{S'}}$. Given the fixed min strategy, the problem faced by the max player resembles the hard MDP instance, so PI requires $\Theta(\sqrt{T})$ iterations by using an argument similar to Theorem~\ref{thm:pi-hard}.
%Now suppose that min-player updates his policy by beginning to choose action $R$ one state earlier. 
%However, in step (2), the SI algorithm plays action $R$ in state $s_{m_{\sqrt{T}}}$, which reduces the value of the state $s_{m_{S'}}'$ by at least $\gamma r_g$. 
%Therefore, the action $a_{S'}$ is no longer the optimal action for the max-player. 
%In the initial iteration of step (1), all actions of other max-player states shall be reset to action $U$ and the action of $s_*$ will be reset to $a_{\sqrt{T}-1}$.
%The above argument continuous until the action of $s_1$ being set to $R$.
%It takes $\Theta(T)$ policy iterations for the max-player to update its policy to the best response to the new min strategy. 
%The total number of policy evaluation needed is $\Theta(T)$, and by the construction we have $\delta_{\max}/\delta_{\min}=\Theta(\sqrt{T})$. Thus we complete the proof.


==> model.tex <==




